Black Hole Fine Structure

In General Relativity, axial and polar black-hole perturbations share identical quasinormal-mode spectra, a property known as isospectrality. New physics can break this degeneracy, producing a spectral splitting analogous to atomic fine structure. We perform a theory-agnostic search for such splitting in gravitational-wave observations. We find no evidence for isospectrality breaking and place a combined $90\%$ upper limit of $<28.5\%$ on the relative frequency splitting. We map these constraints onto several modified-gravity theories, constraining the coupling-lengths to be $\lesssim 28\,\mathrm{km}$.

==> custom_I_symbol.tex <==
\makeatletter
\DeclareRobustCommand{\barredI}{%
  \mathord{\vphantom{I}\mathpalette\@barredI\relax}%
}

\newcommand{\@barredI}[2]{%
  \ooalign{%
    \hidewidth\@barredIbar#1\hidewidth\cr
    $\m@th#1I$\cr
  }%
}

\newcommand{\@barredIbar}[1]{%
  \check@mathfonts
  \ifx#1\displaystyle
    \fontsize{\f@size}{\z@}%
    \def\@barredIbarkern{0.3}%
  \else
    \ifx#1\textstyle
      \fontsize{\f@size}{\z@}
      \def\@barredIbarkern{0.3}%
    \else
      \ifx#1\scriptstyle
        \fontsize{\sf@size}{\z@}
        \def\@barredIbarkern{0.4}%
      \else
        \fontsize{\ssf@size}{\z@}
        \def\@barredIbarkern{0.47}%
      \fi
    \fi
  \fi
  \usefont{OT1}{cmr}{m}{n}%
  \kern-\@barredIbarkern em 
  \raisebox{-.5ex}{\symbol{'26}}%
}
\makeatother
